Metallic Quantum Ferromagnets

This review gives an overview of the quantum phase transition (QPT) problem in metallic ferromagnets, discussing both experimental and theoretical aspects. These QPTs can be classified with respect to the presence and strength of quenched disorder: Clean systems generically show a discontinuous, or first-order, QPT from the ferromagnetic state to a paramagnetic one as a function of some control parameter, as predicted by theory. Disordered systems are much more complicated, depending on the disorder strength and the distance from the QPT. In many disordered materials the QPT is continuous, or second order, and Griffiths-phase effects coexist with QPT singularities near the transition. In other systems the transition from the ferromagnetic state at low temperatures is to a different type of long-range order, such as an antiferromagnetic or a spin-density-wave state. In still other materials a transition to a state with glass-like spin dynamics is suspected. The review provides a comprehensive discussion of the current understanding of these various transitions, and of the relation between experimental and theoretical developments.

==> subsection_II.F.tex <==
\subsection{Superconductivity on the border of itinerant ferromagnetism}
\label{subsubsec:II.F}
%
There are three U-based FM metals which show superconductuvity on the border of itinerant ferromagnetism: 
UGe$_{2}$ (\textcite{Saxena_et_al_2000}), URuGe (\textcite{Aoki_et_al_2001,Yelland_et_al_2011}) 
and UCoGe (\textcite{Huy_et_al_2007a}). It is not the aim of this article to review the coexistence of ferromagnetism
and superconductivity, but we dedicate this brief section to this topic.

==> subsection_II.G.tex <==
%\vfill\eject
\subsection{Summary tables}
\label{subsec:II.G}
%
The experimental results discussed above are summarized in Tables \ref{table:1}, \ref{table:2}, \ref{table:3}, \ref{table:4}.
%%
\vfill\eject
\onecolumngrid
\begin{table*}[!]
\caption{Systems showing a first-order transition. $T_{\text{c}} =$
 Curie temperature, $T_{\text{tc}} =$ tricritical temperature. $\rho_0 =$ 
 residual resistivity. FM = ferromagnet, PM = paramagnet, SC = superconductor. N/A = not applicable;
 n.a. = not available.}
\smallskip
\begin{ruledtabular}
\begin{tabular}{lllllllll}
%\label{table:1}
System $^a$ 
   & Order of 
      & $T_{\text{c}}$/K $^c$
         & magnetic 
            & tuning  
               & $T_{\text{tc}}$/K
                  & wings 
                     & Disorder  
                        & Comments \\

   & Transition $^b$ 
      &                            
         & moment/$\mu_{\text{B}}$ $^d$
            &  parameter 
               &                              
                  & observed  
                     & ($\rho_0/\mu\Omega$cm) $^e$
                        & \\
%\\
\hline\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MnSi$\,^1$
   & 1st$\,^2$ 
      & $29.5$ $\,^3$
         & $0.4$ $\,^3$
            & hyd. press.$\,^2$ 
               & $\approx 10$ $\,^{2,e\alpha}$  
                  & yes$\,^4$
                     & $0.33$ $\,^4$
                        & weak helimagnet;\\
& & & & & & & & exotic phases$\,^{4,6}$ \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
ZrZn$_2$$\,^1$
   & 1st$\,^7$
      & $28.5$ $\,^7$ 
         & $0.17$ $\,^7$
            & hyd. press.$\,^7$
               & $\approx 5$ $\,^7$
                  & yes$\,^7$
                     & $\geq 0.31$ $\,^8$ 
                        & confusing history$\,^1$\\
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
UGe$_2$ $^{10}$
   & 1st$^{11}$ 
      & $52$ $^{12}$
         & $1.5$ $^{12}$
            & hyd. press.$\,^{14,12}$
               & $24$ $^{13}$
                  & yes$\,^{13,12}$
                     & $0.2$ $\,^{14}$
                        & easy-axis FM \\
& & & & & & & & coex. FM+SC$\,^{14}$\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
URhGe$\,^{10}$
   & 1st$\,^{15}$
      & $9.5$ $^{16}$
         & $0.42$ $^{16}$
            &  transverse 
               & $\approx 1$ $\,^{15}$
                  & yes$\,^{15}$
                     & $8$ $\,^{17}$
                        & easy-plane FM\\

   & 
      & 
         & 
            & $B$-field$\,^{18,15}$
               & 
                  & 
                     & 
                        & coex. FM+SC$\,^{16}$ \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
UCoGe$\,^{10}$
   & 1st$\,^{19}$
      & $2.5$ $\,^{19}$
         & $0.03$ $\,^{20}$
            & none 
               & $>2.5$? $\ ^h$
                  & no 
                     & $12$ $\,^{20}$ 
                        & coex. FM+SC$\,^{20}$ \\
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
UCoAl 
   & 1st$\,^{29,r}$
      & $\approx 0\,^{29,s}$
         & $0\,^{29,s}$
            & pressure$\,^{30,31}$
               & $> 11$\,K$\,^{31}$
                 & yes$\,^{31}$
                   & 24$\,^{31}$
                     & large uniaxial\\
& & & & & & & & anisotropy$\,^{30,31}$\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CoS$_2$ 
   & 1st$\,^{21}$ 
      & $122$ $\,^{21}$  
         & $0.84$ $\,^{21}$  
            & hyd. press.$\,^{21}$  
               & $\approx 120$ $\,^{21}$ 
                  & no 
                     & $0.7$ $\,^{21}$
                        & rather high $T_{\text{c}}$\\
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
La$_{1-x}$Ce$_x$In$_2$
   & 1st$\,^{22}$
      & 22 -- 19.5 $\,^{22, i}$ 
         & n.a.
            & composition$\,^{22}$
               & $>22$? $\,^j$
                  & no 
                     & n.a. 
                        & third phase? $\,^{22}$\\
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Ni$_3$Al$\,^{1}$
   & (1st?)$\,^k$
      & 41 -- 15 $\,^l$
         & 0.075 $\,^m$
            & hyd. press.$\,^{24}$ 
               & n.a. 
                  & no 
                     & 0.84 $\,^{23}$
                        & order of trans-\\
& & & & & & & & ition uncertain \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
YbIr$_2$Si$_2$ $^n$
   & 1st$\,^{25}$ 
      & 1.3 -- 2.3 $^o$ 
         & n.a. 
            & hyd. press.$\,^{25}$
               & n.a. 
                  & no 
                     & $\approx 22$ $^p$  
                        & FM order \\
& & & & & & & & suspected$\,^{25}$ \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
YbCu$_2$Si$_2\ ^{n}$
   & 1st$\,^{26}$ 
      & 3.5 -- 6$\,^{26,27,q}$ 
         & 0.16 -- 0.42$\,^{28,r}$
             & hyd. press.$\,^{26-28}$
                & n.a.
                   & no
                      & 220$\,^{28}$
                         &  nature of order\\
& & & & & & & & unclear$\,^{27}$\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
URhAl 
   & (1st?) $\,^t$
      & $\approx 27$ $\,^{32}$
         & $\approx 0.9$ $\,^{32,33}$
            & pressure $\,^{33}$
               & 20 $\,^{33}$
                  & no
                     & $\approx$ 20\,$^{33}$
                        & order of trans-\\
& & & & & & & & ition uncertain\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Sr$_3$Ru$_2$O$_7$
   & 1st$\,^f$
      & 0$\,^g$
         & 0$^{\ g}$
            & pressure$^{\ g}$
               & n.a.
                  & yes$^9$ 
                     & $< 0.5$ $\,^9$
                        & foliated wing tips,\\
& & & & & & & & nematic phase$\,^9$ \\
\hline\\
\multicolumn{9}{l} {$^a$ References in this column refer to review articles, if they exist.\ 
                              $^b$ At the lowest temperature achieved.\ 
                              $^c$ A single value of}\\
\multicolumn{9}{l} {$T_{\text{c}}$, for the default value of the tuning parameter (ambient pressure,
                               zero field) is given if a tricritical temperature has also}\\ 
\multicolumn{9}{l} {been measured. A range of $T_{\text{c}}$, with
                              a corresponding range of the control parameter, is given in all other cases.\ 
                              $^d$ Per formula}\\
\multicolumn{9}{l} {unit unless otherwise noted.\ $^e$ For the highest-quality samples.\ $^f$ Phase diagram not mapped 
                              out completely; the most de-}\\
\multicolumn{9}{l} {tailed measurements show the tips of the wings. See \textcite{Wu_et_al_2011}.\ 
                              $^g$ Paramagetic at ambient pressure. Hydrostatic pres-}\\
\multicolumn{9}{l} {sure drives the system away from FM, uniaxial stress drives it towards FM. See
                               \textcite{Wu_et_al_2011} and references therein, espe-}\\
\multicolumn{9}{l} {cially \textcite{Ikeda_et_al_2000}.\ $^h$ 1st  order transition with no tuning parameter; TCP not accessible.\ 
                              $^i$ For $x = 1.0$ -- $0.9$. \ $^j$ 1st or-}\\
\multicolumn{9}{l} {der for $x=1$, TCP not accessible.\ $^k$ Suspected 1st order transition near $p=80$\,kbar 
                               \cite{Niklowitz_et_al_2005, Pfleiderer_2007}.}\\
\multicolumn{9}{l} {$^l$ For pressures $p=0$ -- $60$\,kbar \cite{Niklowitz_et_al_2005}.\ 
                              $^m$ Per Ni at $p=0$ \cite{Niklowitz_et_al_2005}.\ 
                              $^n$ YbRh$_2$Si$_2$ belongs to the}\\
\multicolumn{9}{l} {same family, but has an AFM phase between the FM and the PM \cite{Yuan_et_al_2006}.\ 
                              $^o$ For pressures $p \approx 8$ -- $10$\,GPa.\ $^p$ For }\\
\multicolumn{9}{l} {a magnetic sample at pressures $p \approx 8$ -- $10$\,GPa. Samples with
                                       $\rho_0$ as low as 0.3$\mu\Omega$cm have been prepared \cite{Yuan_et_al_2006}.}\\
\multicolumn{9}{l} {$^q$ For pressures $p \approx 10$ -- $20$\,GPa.\ $^r$ For pressures $p = 9.4$ -- $11.5$\,GPa.\ 
                              $^s$ PM at zero pressure, FM under uniaxial pressure}\\
\multicolumn{9}{l} {\cite{Ishii_et_al_2003}.\ $^t$ 1st order transition suspected near $p_c \approx 5.3$ GPa \cite{Combier_2013}.\ 
                              $^u$ Disputed by \textcite{Stishov_et_al_2007}; }\\
\multicolumn{9}{l} {see text.}\\
\hline\\
\multicolumn{2}{l}{$^1$ \textcite{Pfleiderer_2007}}  
      & \multicolumn{2}{l}{$^2$ \textcite{Pfleiderer_et_al_1997}} 
            & \multicolumn{2}{l}{$^3$ \textcite{Ishikawa_et_al_1985}} 
                  & \multicolumn{3}{l}{$^4$ \textcite{Pfleiderer_Julian_Lonzarich_2001}} \\
\multicolumn{2}{l}{$^5$ \textcite{Ishikawa_et_al_1976}}  
      & \multicolumn{2}{l}{$^6$ \textcite{Muehlbauer_et_al_2009}} 
            & \multicolumn{2}{l}{$^7$ \textcite{Uhlarz_Pfleiderer_Hayden_2004}} 
                  & \multicolumn{3}{l}{$^8$ \textcite{Sutherland_et_al_2012}} \\
\multicolumn{2}{l}{$^9$ \textcite{Wu_et_al_2011}}  
      & \multicolumn{2}{l}{$^{10}$ \textcite{Aoki_et_al_2011}} 
            & \multicolumn{2}{l}{$^{11}$ \textcite{Huxley_et_al_2001}} 
                  & \multicolumn{3}{l}{$^{12}$ \textcite{Kotegawa_et_al_2011}} \\
\multicolumn{2}{l}{$^{13}$ \textcite{Taufour_et_al_2010}}  
      & \multicolumn{2}{l}{$^{14}$ \textcite{Saxena_et_al_2000}} 
            & \multicolumn{2}{l}{$^{15}$ \textcite{Huxley_et_al_2007}} 
                  & \multicolumn{3}{l}{$^{16}$ \textcite{Aoki_et_al_2001}} \\ 
\multicolumn{2}{l}{$^{17}$ \textcite{Miyake_Aoki_Flouquet_2009}}  
      & \multicolumn{2}{l}{$^{18}$ \textcite{Levy_et_al_2005}} 
            & \multicolumn{2}{l}{$^{19}$ \textcite{Hattori_et_al_2010}} 
                  & \multicolumn{3}{l}{$^{20}$ \textcite{Huy_et_al_2007a}} \\                  
\multicolumn{2}{l}{$^{21}$ \textcite{Sidorov_et_al_2011}}  
      & \multicolumn{2}{l}{$^{22}$ \textcite{Rojas_et_al_2011}} 
            & \multicolumn{2}{l}{$^{23}$ \textcite{Steiner_et_al_2003}} 
                  & \multicolumn{3}{l}{$^{24}$ \textcite{Niklowitz_et_al_2005}} \\     
\multicolumn{2}{l}{$^{25}$ \textcite{Yuan_et_al_2006}}  
      & \multicolumn{2}{l}{$^{26}$ \textcite{Tateiwa_et_al_2014}} 
            & \multicolumn{2}{l}{$^{27}$ \textcite{Winkelmann_et_al_1999}} 
                  & \multicolumn{3}{l}{$^{28}$ \textcite{Fernandez-Panella_et_al_2011}} \\                  
\multicolumn{2}{l}{$^{29}$ \textcite{Andreev_et_al_1985}}  
      & \multicolumn{2}{l}{$^{30}$ \textcite{Ishii_et_al_2003}} 
            & \multicolumn{2}{l}{$^{31}$ \textcite{Aoki_et_al_2011}} 
                  & \multicolumn{3}{l}{$^{32}$ \textcite{Veenhuizen_el_al_1988}} \\    
\multicolumn{2}{l}{$^{33}$ \textcite{Combier_2013}}
      & \multicolumn{2}{l} {  }
            & \multicolumn{2}{l} {  }
                  & \multicolumn{2}{l} {  } \\

               
                  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\end{tabular}
\end{ruledtabular}
\vskip -5mm
\end{table*}
%\nopagebreak
%\noindent
%$^a$ References in this column refer to review articles, if they exist.\quad
%\par\noindent
%$^b$ At the lowest temperature achieved.\quad
%\par\noindent
%$^c$ A single value of $T_{\text{c}}$, for the default value of the tuning parameter (ambient pressure,
%zero field) is given if a tricritical temperature has also been measured. A range of $T_{\text{c}}$, with
%a corresponding range of the control parameter, is given in all other cases.\quad
%\par\noindent
%$^d$ Per formula unit unless otherwise noted.\quad
%\par\noindent
%$^e$ For the highest-quality samples.\quad
%\par\noindent
%$^u$ Disputed by \textcite{Stishov_et_al_2007}; see text.\quad
%\par\noindent
%$^f$ Phase diagram not mapped out completely; the most detailed measurements show
%                               the tips of the wings. See \textcite{Wu_et_al_2011}.\quad
%\par\noindent
%$^g$ Paramagetic at ambient pressure. Hydrostatic pressure drives the
%                                              system away from FM, uniaxial stress drives it towards FM. See
%                                              \textcite{Wu_et_al_2011} and references therein, especially
%                                              \textcite{Ikeda_et_al_2000}.\quad
%\par\noindent
%$^h$ 1st  order transition with no tuning parameter; TCP not accessible.\quad
%\par\noindent
%$^i$ For $x = 1.0$ -- $0.9$. \quad
%\par\noindent
%$^j$ 1st order for $x=1$, TCP not accessible.\quad
%\par\noindent
%$^k$ Suspected 1st order transition near $p=80$\,kbar \cite{Niklowitz_et_al_2005, Pfleiderer_2007}.\quad
%\par\noindent
%$^l$ For pressures $p=0$ -- $60$\,kbar \cite{Niklowitz_et_al_2005}.\quad
%\par\noindent
%$^m$ Per Ni at $p=0$ \cite{Niklowitz_et_al_2005}.\quad
%\par\noindent
%$^n$ YbRh$_2$Si$_2$ belongs to the same family, but has an AFM phase
%                                          between the FM and the PM \cite{Yuan_et_al_2006}.\quad
%\par\noindent
%$^o$ For pressures $p \approx 8$ -- $10$\,GPa.\quad
%\par\noindent
%$^p$ For a magnetic sample at pressures $p \approx 8$ -- $10$\,GPa.
%                                                               Samples with
%                                                               $\rho_0$ as low as 0.3$\mu\Omega$cm have been
%                                                               prepared \cite{Yuan_et_al_2006}.\quad
%\par\noindent
%$^q$ For pressures $p \approx 10$ -- $20$\,GPa.\quad
%\par\noindent
%$^r$ For pressures $p = 9.4$ -- $11.5$\,GPa.\quad
%\par\noindent
%$^s$ PM at zero pressure, FM under uniaxial pressure~\cite{Ishii_et_al_2003}.\quad
%\par\noindent
%$^t$ 1st order transition suspected near $p_c \approx 5.3$ GPa \cite{Combier_2013}.
%\par\noindent
%\begin{tabbing}
%$^1$ \= \textcite{Pfleiderer_2007}\qquad\ \ \ \=
%$^2$ \= \textcite{Pfleiderer_et_al_1997}\qquad\ \ \=
%$^3$ \= \textcite{Ishikawa_et_al_1985}\qquad\ \=
%$^4$ \= \textcite{Pfleiderer_Julian_Lonzarich_2001}\\ 
%$^5$ \> \textcite{Ishikawa_et_al_1976} \>
%$^6$ \> \textcite{Muehlbauer_et_al_2009} \> 
%$^7$ \> \textcite{Uhlarz_Pfleiderer_Hayden_2004} \>
%$^8$ \> \textcite{Sutherland_et_al_2012} \\
%$^9$ \> \textcite{Wu_et_al_2011} \> 
%$^{10}$ \> \textcite{Aoki_et_al_2011} \> 
%$^{11}$ \> \textcite{Huxley_et_al_2001} \> 
%$^{12}$ \> \textcite{Kotegawa_et_al_2011} \\
%$^{13}$ \> \textcite{Taufour_et_al_2010} \> 
%$^{14}$ \> \textcite{Saxena_et_al_2000} \> 
%$^{15}$ \> \textcite{Huxley_et_al_2007} \>
%$^{16}$ \> \textcite{Aoki_et_al_2001}  \\
%$^{17}$ \> \textcite{Miyake_Aoki_Flouquet_2009} \>
%$^{18}$ \> \textcite{Levy_et_al_2005} \> 
%$^{19}$ \> \textcite{Hattori_et_al_2010} \> 
%$^{20}$ \> \textcite{Huy_et_al_2007a} \\
%$^{21}$ \> \textcite{Sidorov_et_al_2011} \>
%$^{22}$ \> \textcite{Rojas_et_al_2011} \> 
%$^{23}$ \> \textcite{Steiner_et_al_2003} \> 
%$^{24}$ \> \textcite{Niklowitz_et_al_2005} \\
%$^{25}$ \> \textcite{Yuan_et_al_2006} \>
%$^{26}$ \> \textcite{Tateiwa_et_al_2014} \>
%$^{27}$ \> \textcite{Winkelmann_et_al_1999} \>
%$^{28}$ \> \textcite{Fernandez-Panella_et_al_2011} \\
%$^{29}$ \> \textcite{Andreev_et_al_1985} \>
%$^{30}$ \> \textcite{Ishii_et_al_2003} \>
%$^{31}$ \> \textcite{Aoki_et_al_2011} \>
%$^{32}$ \> \textcite{Veenhuizen_el_al_1988} \\
%$^{33}$ \> \textcite{Combier_2013} 
%\end{tabbing}
%
%
\vfill\eject
\onecolumngrid
\begin{table*}[!]
\caption{Systems showing a second-order transition. $T_{\text{c}} =$
 Curie temperature, $\rho_0 =$ residual resistivity. QC = quantum critical. First and second group are weakly and strongly 
 disordered, respectively, bulk systems; third group is quasi-1d.}
\smallskip
\begin{ruledtabular}
\begin{tabular}{lllllll}
\label{table:2}
System 
   & Order of 
      & $T_{\text{c}}$/K 
         & magnetic 
            & tuning  
               & Disorder  
                  & Comments \\

   & Transition $^a$ 
      &                            
         & moment/$\mu_{\text{B}}$ $^b$
            &  parameter  
               & ($\rho_0/\mu\Omega$cm) $^c$
                  & \\
%\\
\hline\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Ni$_x$Pd$_{1-x}$ 
   & 2nd$\,^3$
      & 600 -- 7 $\,^f$
         & n.a. & composition$\,^3$
                  & n.a. $^o$
                     & weakly disordered\,$^{13}$ \\
& & & & & & lowest $T_{\text c}$ rather high \\
%\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
(Cr$_{1-x}$Fe$_2$)$_2$B
   & 2nd$\,^{12}$
      & 8 -- 45$\,^n$
         & 0.25 -- 1.4$\,^n$
            & composition
               & 35
                  & disordered\\
%\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hline\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
U$_{2-x}$Re$_x$Si$_2$ 
   & 2nd$\,^{1,2}$
      & 25 -- 2 $\,^d$
         & 0.4 -- 0.03 $\,^2$
            & composition$\,^1$
               & $\approx 100$ $\,^e$
                  & strongly disordered\\
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% YFe$_2$Al$_{10}$
%   & n.a. 
%      &$< 0.09$ $\,^6$
%         & 0 $\,^6$
%            & none
%              & 75 $\,^6$
%                  & strong disorder,\\
% & & & & & & QC fluctuations? $\,^6$ \\
% & & & & & & no ordered phase found \\
% \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Zr$_{1-x}$Nb$_{x}$Zn$_{2}$ 
   & 2nd $\,^{7}$
      & 18 -- 0 $\,^{7,i}$
         & 0 -- 0.08 $\,^{7,i}$
            & composition $\,^{7}$
               & n.a.
                  & disordered, lowest \\
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
SrCo$_{2}$(Ge$_{1-x}$P$_{x}$)$_{2}$ 
   & 2nd $\,^8$  
     & 35 -- 6 $\,^{8,l}$
        & 0.2 -- 0 $\,^{8,l}$ 
           & composition $\,^{8}$
              & n.a.
                 & induced by\\
& & & & & & dimer-breaking \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
U(Rh$_{1-x}$Ru$_{x}$)Ge 
   & 2nd $\,^{9}$
      & $\approx 10$ -- 0 $\,^{9,m}$
         & $\approx 0.1$ -- 0 $\,^{9,m}$
            & composition $\,^{9}$
               & n.a.
                  & disordered \\
& & & & & & no QC fluctuations $\,^{9}$ \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hline\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
YbNi$_4$P$_2$ 
   & 2nd$\,^4$  
      & 0.17 $\,^4$
         & $\approx 0.05$ $\,^4$ 
            & none 
               & 2.6 $\,^4$
                  & quasi-1d\\
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
YbNi$_4$(P$_{1-x}$As$_{x}$)$_2$ 
   & 2nd $\,^5$  
      & 0.17 -- 0.025 $\,^{5,g}$
         & $\approx 0.05$ $\,^5$ 
            & composition 
               & $\approx 5.5$ and 15 $\,^{5,h}$
                  & quasi-1d, disordered
%\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%URhAl 
%   & 2nd $\,^{10,11}$
%      & $\approx 27$ $\,^{10}$
%         & $\approx 0.9$ $\,^{10,11}$
%            & pressure $\,^{11}$
%               & 20 $\,^{11}$
%                  & large uniaxial\\
% & & & & & & anisotropy$\,^{10,11}$\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{tabular}
\end{ruledtabular}
\vskip -3mm
\end{table*}
\nopagebreak
\noindent
$^a$ At the lowest temperature achieved.\quad
%\par\noindent
$^b$ Per formula unit unless otherwise noted.\quad
%\par\noindent
$^c$ For the highest-quality samples.\quad
%\par\noindent
$^d$ For $x=0.6$ -- $0.2$ \cite{Butch_Maple_2009}.\quad
%\par\noindent
$^e$ For $x=0.1$ \cite{Butch_Maple_2010}.\quad
%\par\noindent
$^f$ For $x = 1$ -- $0.027$ \cite{Nicklas_et_al_1999}.\quad
%\par\noindent
$^g$ For $x = 0$ -- $0.08$ \cite{Steppke_et_al_2013}.\quad
%\par\noindent
$^h$ 5.5 for $J \parallel c$ and 15 for $J \perp c$ \cite{Steppke_et_al_2013}.\quad
%\par\noindent
$^i$ For $x = 0$ -- $0.08$ \cite{Sokolov_et_al_2006}.\quad
%\par\noindent
$^l$ For $x = 0.55$ -- $0.35$ \cite{Shuang_et_al_2011}.\quad
%\par\noindent
$^m$ For $x = 0$ -- $0.4$ \cite{Huy_et_al_2007b}.\quad
%\par\noindent
$^n$ For $x = 0.02$ -- $0.05$ \cite{Schoop_et_al_2014}.\quad
%par\noindent
$^o$ Not available for the sample measured; \textcite{Ikeda_1987} has reported values as small as $0.01\,\mu\Omega$cm for
        the Ni concentration range in question.
\medskip\par\noindent
\begin{tabbing}
$^1$ \= \textcite{Bauer_et_al_2005}\qquad\qquad\ \=
$^2$ \= \textcite{Butch_Maple_2009}\qquad\ \=
$^3$ \= \textcite{Nicklas_et_al_1999}\qquad\ \=
$^4$ \= \textcite{Krellner_et_al_2011} \\ 
%
$^5$ \> \textcite{Steppke_et_al_2013} \>
% $^6$ \> \textcite{Park_et_al_2011} \>
$^7$ \> \textcite{Sokolov_et_al_2006} \>
$^8$ \> \textcite{Shuang_et_al_2011} \>
$^9$ \> \textcite{Huy_et_al_2007b} \\%
$^{10}$ \> \,\textcite{Veenhuizen_el_al_1988} \>
$^{11}$ \> \,\textcite{Combier_2013} \>
$^{12}$ \> \,\textcite{Schoop_et_al_2014} \>
$^{13}$ \> \,\textcite{Ikeda_1987}
\end{tabbing}
\medskip
%\hrule
\bigskip
%\twocolumngrid
\vfill\eject
%
\onecolumngrid
\begin{table*}[!]
\caption{System showing change into a spin-density-wave (SDW) or antiferromagnetic (AFM) order. $T_{\text{N}} =$
 N\'eel temperature, $\rho_0 =$ residual resistivity. QC = quantum critical.}
\smallskip
\begin{ruledtabular}
\begin{tabular}{llllllll}
\label{table:3}
System 
   & Order of 
      & $T_{\text{c}}$/K 
         & $T_{\text{N}}$/K 
            & magnetic 
               & tuning  
                  & Disorder  
                     & Comments \\

   & Transition $^a$ 
      &        
         &                    
            & moment/$\mu_{\text{B}}$ $^b$
               &  parameter  
                  & ($\rho_0/\mu\Omega$cm) $^c$
                     & \\
%\\
\hline\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CeRu$_{2}$(Ge$_{1-x}$Si$_x$)$_{2}$ 
   & 2nd$\,^1$
      & 2.5 -- 8 $\,^1$
         & 1 -- 10 $\,^1$
            & n.a.
               & comp./press.$\,^1$
                  & n.a.
                     & dis., lowest \\
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Nb$_{1-y}$Fe$_{2+y}$ 
   & 2nd$\,^{2,3}$
      & 6 -- 72 $\,^d$
         & 2.8 -- 32 $\,^e$
            & $\approx 0.02$ $\,^{2}$ 
               & comp.$\,^3$
                  & 5.5 $\,^3$
                     & dis., lowest \\
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Yb(Rh$_{1-x}$Co$_{x})_{2}$Si$_2$ 
   & 2nd$\,^{4,6}$
      & 1.3 $\,^{6,f}$
         & 0.07 -- 1.2 $\,^4$
            & 0.002 -- 0.1 $\,^{5,6,g}$
               & comp./press.$\,^{4,7,8}$
                  & 0.5 -- 10 $\,^{4,9}$
                     & dis., lowest \\
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CeRuPO 
   & 2nd $\,^{10,11}$
      & 15 -- 11 $\,^{11,12,h}$
         & 10 -- 1 $\,^{11,12,h}$
            & 1.2 $\,^{10}$
               & pressure $\,^{11,12,h}$
                  & $\approx 30\,^{12}$
                     & dis., lowest \\
& & & & & & & \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CeRu$_{1-x}$Fe$_{x}$PO 
   & 2nd $\,^{13}$  
     & 15 -- 0.3 $\,^{13}$
        & $\approx 0.5$ -- $0 \,^{13}$
          & 1.2 $\,^{10}$
            & comp. 
              & n.a.
                 & dis., quasi-2d$\,^{14}$\\
& & & & & & & QC fluctuations \\
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CeFeAs$_{1-x}$P$_{x}$O 
   & 2nd $\,^{15,16}$
      & $\approx 10$ -- 6 $\,^{15,16,i}$
         & $\approx 3$ $\,^{15,16,l}$
            & 0.95 -- 0 $\,^{15}$
               & comp. $\,^{15,16,i,l}$
                  & n.a.
                     & unclear\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{tabular}
\end{ruledtabular}
\vskip -3mm
\end{table*}
\nopagebreak
\noindent
$^a$ At the lowest temperature achieved.\quad
%\par\noindent
$^b$ Per formula unit unless otherwise noted.\quad
%\par\noindent
$^c$ For the highest-quality samples.\quad
%\par\noindent
$^d$ For $y = 0.007$ -- $0.04$ \cite{Brando_et_al_2008,Moroni_et_al_2009}.\quad
%\par\noindent
$^e$ For $y = -0.01$ -- $0.015$ \cite{Brando_et_al_2008,Moroni_et_al_2009}.\quad
%\par\noindent
$^f$ For Yb(Rh$_{0.73}$Co$_{0.27}$)$_2$Si$_2$ (\textcite{Lausberg_et_al_2013}).\quad
%\par\noindent
$^g$ 0.002 $\mu_{\text{B}}$ for YbRh$_2$Si$_2$ (\textcite{Ishida_et_al_2003}) 0.1 $\mu_{\text{B}}$ for Yb(Rh$_{0.73}$Co$_{0.27}$)$_2$Si$_2$ (\textcite{Lausberg_et_al_2013}).\quad
%\par\noindent
$^h$ FM for $0 \leq p \leq 0.8$\,GPa and AFM for $0.8 \leq p \leq 2.8$\,GPa \cite{Macovei_2010,Kotegawa_et_al_2013}.\quad
%\par\noindent
$^i$ For $x = 0.4$ -- $0.8$ \cite{Luo_et_al_2010,Jesche_et_al_2012}.\quad
%\par\noindent
$^l$ For $x = 0.9$ (\textcite{Luo_et_al_2010}).
\medskip\par\noindent
\begin{tabbing}
$^1$ \= \textcite{Suellow_et_al_1999}\qquad\ \=
$^2$ \= \textcite{Brando_et_al_2008}\qquad\ \=
$^3$ \= \textcite{Moroni_et_al_2009} \=
$^4$ \= \textcite{Klingner_et_al_2011} \\ 

$^5$ \> \textcite{Ishida_et_al_2003} \>
$^6$ \> \textcite{Lausberg_et_al_2013} \>
$^7$ \> \textcite{Mederle_et_al_2001} \>
$^8$ \> \textcite{Knebel_et_al_2006} \\ 
%
$^9$ \> \textcite{Krellner_et_al_2009} \>
$^{10}$ \> \textcite{Krellner_et_al_2007} \>
$^{11}$ \> \textcite{Macovei_2010} \>
$^{12}$ \> \textcite{Kotegawa_et_al_2013}\\
%
$^{13}$ \> \textcite{Kitagawa_et_al_2012} \>
$^{14}$ \> \textcite{Kitagawa_et_al_2013} \>
$^{15}$ \> \textcite{Luo_et_al_2010} \>
$^{16}$ \> \textcite{Jesche_et_al_2012}
\end{tabbing} 
\medskip
%\hrule
\bigskip
%\twocolumngrid
\vfill\eject

%
\onecolumngrid
\begin{table*}[!]
\caption{System showing short-range order or spin-glass (SG) freezing. $T_{\text{g}} =$
 freezing temperature, $\rho_0 =$ residual resistivity. QC = quantum critical. QGP = quantum Griffiths phase.}
\smallskip
\begin{ruledtabular}
\begin{tabular}{llllllll}
\label{table:4}
System 
   & Order of 
      & $T_{\text{c}}$/K 
         & $T_{\text{g}}$/K 
            & magnetic 
               & tuning  
                  & Disorder  
                     & Comments \\

   & Transition $^a$ 
      &        
         &                    
            & moment/$\mu_{\text{B}}$ $^b$
               &  parameter  
                  & ($\rho_0/\mu\Omega$cm) $^c$
                     & \\
%\\
\hline\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CePd$_{1-x}$Rh$_x$ 
   & 2nd$\,^1$
      & 6.6 -- 3 $\,^{1,2,d}$
         & 3 -- 0 $\,^{1,2,e}$
            & n.a.
               & comp.$\,^{1,2}$
                  & n.a.
                     & disordered \\
& & & & & & & QGP \\
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CeFePO
   & SG$\,^{3}$
      & n.a.
         & 0.9 $\,^{3}$
            & n.a.
               & --
                  & $\approx 20$ $^{3,4,f}$
                     & not disordered \\
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
UNiSi$_{2}$
   & 2nd$\,^{5}$
      & 95 $^{5,6,7}$
         &  $< 15$ $\,^{5,g}$
            & 1.2 $\,^{6}$
               & pressure $\,^{5}$
                  & $\approx 25$ $^{5}$
                     & not disordered \\
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
UNi$_{1-x}$Co$_x$Si$_2$ 
   & 2nd$\,^7$
      & 95 -- 8.6 $\,^{7,h}$
         & 6 $\,^{7,i}$
            & n.a.
               & comp.$\,^7$
                  & n.a.
                     & disordered \\
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
U$_{1-x}$Th$_x$NiSi$_2$ 
   & 2nd$\,^8$
      & 95 -- 29 $\,^{8,l}$
         & 29 -- $\approx 4$ $\,^{8,m}$
            & n.a.
               & comp.$\,^8$
                  & n.a.
                     & disordered \\
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Sr$_{1-x}$Ca$_x$RuO$_3$ 
   & 2nd$\,^9$
      & $\approx 100$ -- 40 $\,^{9,n}$
         & $\approx 40$ -- $\approx 5$ $\,^{9,o}$
            & 1 -- 0
               & comp. on a single film$\,^9$
                  & n.a.
                     & disordered \\
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Ni$_{1-x}$V$_x$ 
   & 2nd$\,^{10}$
      & 633 -- $\approx 30$ $\,^{10,p}$
         & $\approx 30$ -- $0.2$ $\,^{10,q}$
            & 0.6 -- 0
               & comp.$\,^{10}$
                  & n.a.
                     & disordered \\
& & & & & & & QGP \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CeTi$_{1-x}$V$_x$Ge$_{3}$ 
   & 2nd$\,^{11,12}$
      & 14 -- 2.8$\,^{11,12}$
         & n.a.
            & 1.5$\,^{12}$
               & comp.$\,^{12}$
                  & 22$\,^{12,r}$
                     & disordered \\
& & & & & & & QGP \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{tabular}
\end{ruledtabular}
\vskip -3mm
\end{table*}
\nopagebreak
\noindent
$^a$ At the lowest temperature achieved.
\par\noindent
$^b$ Per formula unit unless otherwise noted.
\par\noindent
$^c$ For the highest-quality samples.
\par\noindent
$^d$ For $x = 1$ -- $0.6$ (\textcite{Sereni_et_al_2007})
\par\noindent
$^e$ For $x = 0.6$ -- $0.9$ (\textcite{Sereni_et_al_2007,Westerkamp_et_al_2009})
\par\noindent
$^f$ High $\rho_{0}$ not due to disorder but to strong FM fluctuations
\par\noindent
$^g$ Nature of the phase not clear, possibly weakly ferromagnetic (\textcite{Sidorov_et_al_2011a}) \tred{(possibly, move to table III)}
\par\noindent
$^h$ For $x = 0$ -- $0.96$ (\textcite{Pikul_et_al_2012b})
\par\noindent
$^i$ For $x = 0.98$ (\textcite{Pikul_et_al_2012b})
\par\noindent
$^l$ For $x = 0$ -- $0.7$ (\textcite{Pikul_et_al_2012a})
\par\noindent
$^m$ For $x = 0.7$ -- $0.9$ (\textcite{Pikul_et_al_2012a})
\par\noindent
$^n$ For $x = 0.15$ -- $0.38$ (\textcite{Demko_et_al_2012})
\par\noindent
$^o$ For $x = 0.38$ -- $0.52$ (\textcite{Demko_et_al_2012})
\par\noindent
$^p$ For $x = 0$ -- $0.105$ (\textcite{Ubaid-Kassis_et_al_2010})
\par\noindent
$^q$ For $x = 0.11$ -- $0.1225$ (\textcite{Ubaid-Kassis_et_al_2010})
\par\noindent
$^r$ For CeTiGe$_{3}$ (\textcite{Kittler_et_al_2013})
\medskip\par\noindent
\begin{tabbing}
$^1$ \= \textcite{Sereni_et_al_2007}\qquad\qquad\ \ \ \=
$^2$ \= \textcite{Westerkamp_et_al_2009}\ \ \ \=
$^3$ \= \textcite{Lausberg_et_al_2012a}\qquad\ \=
$^4$ \= \textcite{Jesche_2011} \\
$^5$ \= \textcite{Sidorov_et_al_2011a} \>
$^6$ \= \textcite{Das_et_al_2000} \>
$^7$ \> \textcite{Pikul_et_al_2012b} \\
$^8$ \> \textcite{Pikul_et_al_2012a} \>
$^9$ \> \textcite{Demko_et_al_2012} \>
$^{10}$ \> \textcite{Ubaid-Kassis_et_al_2010} \>
$^{11}$ \> \textcite{Manfrinetti_et_al_2005} \\
$^{11}$ \> \textcite{Kittler_et_al_2013}
\end{tabbing}
\medskip
%\hrule
\bigskip
\newpage
\twocolumngrid
\vfill\eject
